Entropy Guided Spectrum Based Bug Localization Using Statistical Language Model

Locating bugs is challenging but one of the most important activities in software development and maintenance phase because there are no certain rules to identify all types of bugs. Existing automatic bug localization tools use various heuristics based on test coverage, pre-determined buggy patterns, or textual similarity with bug report, to rank suspicious program elements. However, since these techniques rely on information from single source, they often suffer when the respective source information is inadequate. For instance, the popular spectrum based bug localization may not work well under poorly written test suite. In this paper, we propose a new approach, EnSpec, that guides spectrum based bug localization using code entropy, a metric that basically represents naturalness of code derived from a statistical language model. Our intuition is that since buggy code are high entropic, spectrum based bug localization with code entropy would be more robust in discriminating buggy lines vs. non-buggy lines. We realize our idea in a prototype, and performed an extensive evaluation on two popular publicly available benchmarks. Our results demonstrate that EnSpec outperforms a state-of-the-art spectrum based bug localization technique.

==> Makefile <==
# $Id: Makefile 1833 2006-06-19 21:51:36Z witchel $

.SUFFIXES: .fig .dvi .ps .pdf

VERSION = 0.0

#----------------------------------------------------------------------
# Source files.  Edit these variables for each new paper.
#----------------------------------------------------------------------

name = main

all: pdf bib

#----------------------------------------------------------------------
# LaTeX commands.
#----------------------------------------------------------------------

%.dvi:%.tex
	pdflatex $<

dvi: $(name).tex *.tex
	pdflatex $<

rub: $(name).tex 
	rubber -Wrefs -Wmisc $(name)

twice:
	pdflatex $(name)
	pdflatex $(name)

bib:
	bibtex $(name)
	pdflatex $(name)
	pdflatex $(name)


latex_junk = 	$(name).dvi \
		*.aux \
		*.log \
		$(name).blg \
		$(name).toc \
		psfig.aux \
		*.bbl \
		*.pdfsync

#----------------------------------------------------------------------
# Postscript/PDF generation.
#----------------------------------------------------------------------

$(name).ps:
ps: $(name).dvi *.tex
	latex $(name).tex && latex $(name).tex
	$(DVIPS) -P pdf -t letter -o $(name).ps $(name).dvi

summary: summary.dvi

#DVIPS = dvips
DVIPS = dvips

%.ps:%.dvi
	$(DVIPS) -P pdf -t letter -o $@ $<

%.ps2:%.dvi
	$(DVIPS) -t letter -o ps2.tmp -p 2 $<
	mpage -2 -P ps2.tmp > $@
	rm ps2.tmp

pdf: 
	pdflatex $(name).tex

# DISTILL = distill
DISTILL_FLAGS = -embedallfonts on -maxsubsetpct 100

DISTILL = ps2pdf
#DISTILL_FLAGS =

%.pdf:%.ps
	$(DISTILL) $(DISTILL_FLAGS) $<

#----------------------------------------------------------------------
# Document previewers.
#----------------------------------------------------------------------

x:
	xdvi -s 5 $(name) &

gv: $(name).ps
	ghostview $(name).ps &


# Garbage files.
junk = $(latex_junk) *.ps *.pdf *.out


#----------------------------------------------------------------------
# Miscellaneous.
#----------------------------------------------------------------------

tags:
	etags $(latex_files)

clean:
	rm -f $(junk)

count:
	wc $(latex_files)


==> aucec_5.tex <==
\begin{center}
\begin{figure*}
\subfloat[]{%
  \begin{minipage}{\linewidth}
  \includegraphics[width=.3\linewidth]{defects4j_graph/chart_5}\hfill
  \includegraphics[width=.3\linewidth]{defects4j_graph/lang_5}\hfill
  \includegraphics[width=.3\linewidth]{defects4j_graph/time_5}%
  \end{minipage}%
  }
\caption{Effect of \LM while inspecting 5\% SLOC}
\label{fig:aucec_5}
\end{figure*}
\end{center}

==> method_bck.tex <==
%!TEX root = main.tex
\begin{figure*}[!htpb]
\centering
\includegraphics[width=\textwidth]{images/schema.png}
\caption{\textbf{\small \tool Workflow}}
\label{fig:schema}
\end{figure*}

\section{Study Method}% and Experiments}
\label{sec:method}

In this section, we describe the dataset we studied and the analysis methods we used to answer our research
questions.

\subsection{Study Subject}
\label{subsec:study_subject}

We used two publicly available bug dataset: \defj~\cite{just2014defects4j} and 
\mbug~\cite{le2015manybugs} (see Table~\ref{tab:ssubj}).  \defj dataset contains $5$ open source projects with $321$K lines of code, $357$ reproducible bugs, and $20$K total number of tests. All the \defj projects are written in Java. We also studied $5$ projects from \mbug benchmark dataset~\cite{le2015manybugs}. These are medium to large open source C projects, with total $4459$K lines of code, $160$ reproducible bugs, and $9262$ total test cases. In both datasets, each bug is associated with a buggy and its corresponding fix program versions. There are some failing test cases that reproduce the bugs in the buggy versions, while after the fixes all the test cases pass. The dataset also provides APIs for instrumentation and recording program execution traces.

\input{tables/dataset}

\subsection{Data Collection}
\label{subsec:dc}

Here we describe how we identified the buggy lines in a buggy program version. 
%\subsubsection{Bug Annotation}
%\label{subsec:bug_annot}





{\em Annotating buggy program statements.} We compared each buggy program version with its corresponding fixed version; the lines that are deleted or modified in the buggy version are annotated as buggy program statements. To 
get the differences between two program versions, we used \defj APIs for \defj dataset.~\sk{How did you get differences of \mbug dataset?} 

We notice that some bugs in \defj dataset\sk{what about \mbug?} are caused due to the error of omission\textemdash tests fail due to missing features/functionalities in the buggy version. Fixing these bugs do not require deleting or modifying program statements in the buggy version, but adding new lines in the fixed version. In such cases, we cannot trivially annotate any of the existing lines in the buggy version as `buggy.' We filter out such bugs from further consideration, as our goal in this work to locate existing buggy lines, as opposed to detecting error of omission.~\ripon{Ripon, I do not think we need to cite example, as it is trivial. What do you think?} Table~\ref{tab:ssubj} shows the total number of buggy lines per each \defj project. 

% Next challenge of this project is annotating the buggy lines to train the model. From Defects4j API, we get the difference between buggy version and corresponding fix versions. Out study shows that a large portion of the bug are fixed by inserting new lines or blocks of code. For example, in Figure \ref{fig:bug_annot_ins}, code difference of buggy and fix version of Bug $30$ of Project \textit{Lang} is showed. Although, this bug causes test cases to fail, this is patched by introducing new lines. None of the existing lines are changed or deleted. Hence, we cannot trivially annotate any of the existing lines in buggy version of the code as buggy. 

% \begin{figure}[!htpb]
% \centering
% \includegraphics[width=0.5\textwidth]{images/bug_annot_insert.png}
% \caption{Bug$30$ of Project Lang fixed by inserting lines}
% \label{fig:bug_annot_ins}
% \end{figure}
% \begin{figure}[!htpb]
% \centering
% \includegraphics[width=0.5\textwidth]{images/bug_annot_change.png}
% \caption{\textbf{\small Bug$30$ pf Project Lang fixed by Changing}}
% \label{fig:bug_annot_change}
% \end{figure}

% On the other hand, Figure \ref{fig:bug_annot_change} shows the a fix, where the buggy line is fixed by a change. Logically we can say, there was something wrong with this line in the buggy version, so we can annotate that line as buggy. 
%Using this bug annotation strategy, number of lines annotated as buggy for the projects of \defj are illustrated in table \ref{tbl:buggy_lines}.

% \begin{table}[!htpb]
% \scriptsize
% \centering
% \caption{\textbf{\small Number of buggy lines for \defj dataset}}
% \label{tbl:buggy_lines}
% \begin{tabular}{l|c|c}
% Project		&	\#buggy lines & \#buggy lines \\
%     		&	(\defj) & (\defj + evolution)\\

% \toprule
% \chart		&	22 & 32\\
% \lang	&	50 & 230\\
% \closure	&	64 & 586\\
% \maths		& 	38 & 816\\
% \jtime			&	46 & 97\\
% \bottomrule
% Total		&	220 & 1761\\
% \end{tabular}

% \end{table}

Obviously, this is a very small number to work on. So we searched on those project evolution history for more bugs. We adopted the similar strategy described in \textit{Ray et al.}\cite{ray2016naturalness} First, we searched project repository for bug fix commit messages based on special keywords in commit messages. As described in Mockus ~\etal~\cite{mockus2000identifying}, we searched commit messages containing error related keywords such as `error', `bug', `fix', `issue', `mistake', `flaw', `defect' etc. Lines changed or deleted on those commits are marked as buggy. Then the commits those had introduced these buggy lines are located. then using `git blame' with `--reverse' option, those lines are located in the nearest snapshot of the originating commit. ~\sk{Elaborate this.} From project evolution history, we found other bugs to train our model on. And total number of buggy lines found are also shown in table \ref{tbl:buggy_lines}.

Another approach is very popular in literature, which injects faults in the software system for testing \cite{gunneflo1989evaluation,segall1995fiat}. But in our model, we heavily rely on the naturalness of the code. And, injected code will violate the hypotheses of code being natural. So, we did not adopt that approach.

\subsubsection{Data Filtering}
\label{subsec:data_filtering}
We are dealing with fault localization. We know there are faults because, some of the test cases failed. There are some lines in a project which is not even been touched by any of the failing test cases. So we exclude those lines from consideration. 
Obviously, some of the buggy lines from project evolution are excluded. The reason for that is, although we have sufficient failing test cases for all of the bugs given by defects4j, we do not have sufficient test cases to identify all the buggy lines identified from the project evolution. ~\sk{Is it also done for manybugs dataset.}
Number of buggy lines after this filtering is shown in table \ref{tbl:after_filtering} 
\begin{table}[h]
\centering
\begin{tabular}{c|c|c}
Project name		&	\#Total Lines &  \#Buggy Lines\\
\hline
\hline
jfree-\textbf{Chart}		&	2311 & 30\\
Commons-\textbf{Lang}		&	29525 & 249\\
\textbf{Closure}-compiler	&	4504 & 134\\
Commons-\textbf{Math}		& 	2793 & 577\\
Joda-\textbf{Time}			&	588 & 46\\
\hline
Total		&	39721 & 1035\\
\end{tabular}
\caption{Number of lines to be considered and number of buggy lines}
\label{tbl:after_filtering}
\end{table}

\subsection{Methodology}
\label{subsec:method}


\subsubsection{Program Spectra Generation}
\label{subsec:program_spectra}

First, we extracted the Test Classes and Test methods from the Project Source codes. Then, we run our test cases and recorded the execution trace of different passing and failing test cases. We also recorded the passing status of the corresponding test case. 

From there we calculated line 4 values$(e_p, e_f, n_p, n_f)$ described in Section \ref{sec:intro}. With these 4 values, we generated 25 ranking matrices in the state of the art described in \textit{Xuan et al.} \cite{xuan2014learning}. We used these 25 ranking metrics as our considered features. These values are referred to as Spectrum based features in the context of this report.
%\begin{table}[h]
%\label{tbl:rank_metrics}
%\begin{tabular}{|c|c||c|c|}
%\hline
%Ranking Metric & Formula & Ranking Metric & Formula\\
%\hline
%\hline
%Tarantula & $\frac{\frac{e_f}{e_f+n_f}}{\frac{e_f}{e_f+n_f} + \frac{e_p}{e_p+n_p}}$ & Ochiai & $\frac{e_f}{\sqrt{(e_f+e_p)(e_f+n_f)}}$\\
%\hline
%Jaccard & $\frac{e_f}{e_f+e_p+n_f}$ & RusselRao & $\frac{e_f}{e_p + e_f + n_p + n_f}$\\
%\hline
%S$\phi$orensenDice & $\frac{2e_f}{2e_f + e_p + n_f}$ & Kulczynski1 & %$\frac{e_f}{n_f+e_p}$\\
%\hline
%SimpleMatching & $\frac{e_f+n_p}{n_p+n_f+e_p+e_f}$ & M1 & $\frac{e_f + n_p}{n_f+e_p}$\\
%\hline
%M2 & \\
%\hline
%\end{tabular}
%\end{table}

\subsubsection{Entropy Generation}
\label{sebsec:entropy_gen}
For generating entropy we adopted the \textit{\$-gram} model proposed by \textit{Tu et al.}\cite{tu2014localness}. For every line in source code we, calculated $3$ entropy values. Those are:
\begin{itemize}
\item \textbf{Forward Entropy $(E_f)$}: This entropy is calculated by parsing the file from begin to end, \textit{i.e.} considering the token sequence as it is in the source file.
\item \textbf{Backward Entropy $(E_b)$}: This entropy is calculated by parsing the file in reverse order, \textit{i.e.} considering the token sequence from end to the begin of file. 
\item \textbf{Average Entropy $(E_a)$}: This entropy value is calculated as the average of $E_f$ and $E_b$.
\end{itemize}
We used these 3 values as our feature for algorithm. In this report, we refer to this values as \textit{Entropy based features}.




Inspired by the approach described at Li ~\etal~\cite{li2007mcrank}, we annotated all lines in our train dataset with a relevance score of being buggy. Intuitively, this score should by higher for the actual buggy lines. To maintain clarity, we maintained one relevance score for all the buggy lines and one score for non-buggy lines. Let $R_b$ be the relevance score of buggy lines, and $R_g$ be the relevance score for good lines.
We chose $R_b$ and $R_g$ such that $R_b > R_g$.
Impact of assigning different scores for buggy and/or non-buggy lines is beyond the scope of this research.

We represent each line $l_i$ in the training code corpus as a tuple, $<Sp_i,En_i,R_i>$, where $SP_i$ are the spectrum based suspiciousness scores, $EN_i$ are the Entropy scores, and $R_i \in \{R_b, R_g\}$ is the relavenace score.Themn, we pass the whole corpus to a learning machine, which learns the probability distribution $P(R_i|Sp_i,En_i)$ of the relevance scores given the feature values. While the model is in test phase, for each line $L_i$ in test corpus, we compute supiciousness score based on equation ~\ref{eqn:proba_suspiciousness_score}
\begin{equation}
\label{eqn:proba_suspiciousness_score}
\begin{split}
Susp_{L_i} = f(R_b) &* P(R_b|Sp_{L_i},En_{L_i})\\
&+ f(R_g) * P(R_b|Sp_{L_i},En_{L_i})
\end{split}
\end{equation}
Here, $f(R_i)$ is monotonically increasing function. To keep things simple, we used identity function \textit{i.e.} $f(R_b) = R_b$ and $f(R_g) = R_g$, which is of course monotonically increasing function. Choosing this identity function will transform equation ~\ref{eqn:proba_suspiciousness_score} into
\begin{equation}
\label{eqn:expected_value_suspiciousness}
\begin{split}
Susp_{L_i} &= \sum_{R_i \in \{R_b, R_g\}}{R_i * P(R_i|Sp_{L_i},En_{L_i})} \\
&= \mathbb{E}[R_i|Sp_{L_i}, En_{L_i}] 
\end{split}
\end{equation}
This is the expected relevance score for a line being buggy. We evaluated our approach based on this score. 
\subsection{Evaluation Metric}
\label{sunsec:evaluation_metric}
Todo: Add description of evaluation metric. 


\subsection{Random Forest Algorithm}
\label{subsec:randomforest}
Random Forest(RF) is an ensemble learning technique developed by Breiman(2001)\cite{breiman2001random} based on a combination of a large set of decision trees. Each tree is trained by selecting a random set of variables and a random sample from the training dataset (\textit{i.e.}, the different spectrum scores and/or entropies by \$-gram model). In addition to learning the discrimination function for classification task, RF also learns class conditional probability distribution of train dataset. Additionally, RF algorithm learns the importances for different features for discrimination. In this work, we leveraged the  feature importance(i.e. importances of different \textit{suspiciousness} scores and \textit{entropy} based features)  and class conditional probability distribution learned by RF algorithms. As described by Provost \etal~\cite{provost2003tree}, we used the class conditional probability estimation of a test program line as the suspiciousness score. 

\subsection{Training}
\label{subsec:training}
Having the pre-processing described in section \ref{subsec:program_spectra},\ref{subsec:bug_annot},and\ref{subsec:data_filtering} done, we train our model using simplified Random Forest Algorithm, where we learn the relative importances of the features to classify the data into buggy and non-buggy version, and also we learned the class conditional probability distribution of the training data.
